Determination of $\alpha_{S}$ beyond NNLO using event shape averages

We consider a method for determining the QCD strong coupling constant using fits of perturbative predictions for event shape averages to data collected at the LEP, PETRA, PEP and TRISTAN colliders. To obtain highest accuracy predictions we use a combination of perturbative ${\cal{O}}(\alpha_{S}^{3})$ calculations and estimations of the ${\cal{O}}(\alpha_{S}^{4})$ perturbative coefficients from data. We account for non-perturbative effects using modern Monte Carlo event generators and analytic hadronization models. The obtained results show that the total precision of the $\alpha_{S}$ determination cannot be improved significantly with the higher order perturbative QCD corrections alone, but primarily requires a deeper understanding of the non-perturbative effects.

==> Makefile <==
#ulimit -u 10000
latexfile=MOM
newname?=MOM
STYLE=arxiv

LATEX=  lualatex -halt-on-error -shell-escape -enable-write18
LATEX=  pdflatex -halt-on-error -shell-escape -enable-write18
BIBTEX=bibtex


ifeq ($(STYLE),draft)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-draft.tex 
endif

ifeq ($(STYLE),arxiv)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-arxiv.tex 
endif

ifeq ($(STYLE),epjc)
	STYLE_SPECIFIC_FILES=svjour.cls  svepj.clo $(latexfile)-epjc.tex 
endif


all: $(latexfile)-$(STYLE).pdf

tar:  Makefile $(figures) $(constanttables) $(tables) $(latexfile).bst $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-val.tex $(latexfile)-tab.tex  $(latexfile)-val.tex  $(STYLE_SPECIFIC_FILES)
	rm -rf TAR
	mkdir -p TAR
	cp Makefile  $(latexfile).bst $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-def.tex $(latexfile)-txt.tex $(latexfile)-tab.tex  $(latexfile)-val.tex   $(STYLE_SPECIFIC_FILES) TAR
ifeq ($(STYLE),epjc)
	cp $(figures) TAR/
else
	mkdir -p TAR/Figures
	cp $(figures) TAR/Figures
endif
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/*tex	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/Makefile
	sed -i 's@^STYLE.*@STYLE='$(STYLE)'@g' TAR/Makefile
	sed -i '/@artic/achecked={2},'     TAR/*bib	
	sed -i '/@inproceed/achecked={2},' TAR/*bib	
	sed -i '/@phdthesis/achecked={2},' TAR/*bib	

ifeq ($(STYLE),epjc)
	sed -i 's@\[htbp\]@@g' TAR/$(latexfile)-tab.tex
	sed -i 's@c|@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@|c@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@}|@}@g' TAR/$(latexfile)-tab.tex
endif
	
	mv TAR/$(latexfile).bst TAR/$(newname).bst 
	mv TAR/$(latexfile).bib TAR/$(newname).bib 
	mv TAR/$(latexfile)-$(STYLE).tex TAR/$(newname)-$(STYLE).tex
ifeq ($(STYLE),epjc)
	sed -i 's@Figures/@@g' TAR/Makefile
endif
	mv TAR/$(latexfile)-txt.tex TAR/$(newname)-txt.tex
	mv TAR/$(latexfile)-abs.tex TAR/$(newname)-abs.tex
	mv TAR/$(latexfile)-def.tex TAR/$(newname)-def.tex
	mv TAR/$(latexfile)-tab.tex TAR/$(newname)-tab.tex
	cat TAR/$(latexfile)-val.tex | grep [:0-9:] > TAR/$(newname)-val.tex
	rm -f TAR/$(latexfile)-val.tex
ifeq ($(STYLE),arxiv)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
ifeq ($(STYLE),epjc)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
	tar -zcvf   $(newname).tar.gz -C TAR . 
	rm -rf $(newname).zip; cd TAR; zip ../$(newname).zip ./*/* ./*; cd ..

	rm -rf TAR


figures=  Figures/figC1-figure0.pdf   Figures/figC1NNLO-figure0.pdf   \
           Figures/figCorrSZ-figure0.pdf     \
           Figures/fighadC1-figure0.pdf     \
           Figures/fighadoneminusT1-figure0.pdf   \
           Figures/figMCC1-figure0.pdf   \
           Figures/figMConeminusT1-figure0.pdf   \
           Figures/figoneminusT1-figure0.pdf   
tables=
constanttables=


$(latexfile)-$(STYLE).pdf :  $(figures) $(constanttables) $(tables) $(latexfile).bst\
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex\
                       $(latexfile)-val.tex $(STYLE_SPECIFIC_FILES)
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
ifeq ($(STYLE),epjc)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
ifeq ($(STYLE),arxiv)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
	sed -i 's@Collaboration@Coll\.@g'  $(latexfile)-$(STYLE).bbl
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)

pdf : $(latexfile)-$(STYLE).pdf

$(latexfile).rws: $(latexfile)-dict.txt
	aspell --lang=en create master ./$(latexfile).rws < ./$(latexfile)-dict.txt

spell: $(latexfile).rws
	for a in $$(ls -1 $(latexfile)-*.tex ../EPJC/*/Answer*tex); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-extra-dicts=./$(latexfile).rws  -t --dont-tex-check-comments -d en_GB -c $$a ;\
	done

clean :
	rm -f *.aux
	rm -f *.lof
	rm -f *.out
	rm -f *.lot
	rm -f *.bbl
	rm -f *.l4l
	rm -f *.log
	rm -f *.blg
	rm -f *.ilg
	rm -f *.aux
	rm -f $(latexfile)*.dvi
	rm -f $(latexfile)*.ps
	rm -f $(latexfile)*.pdf
	rm -f *.toc
	rm -f *.idx
	rm -f *.ind
	rm -f *.nav
	rm -f *.snm


